Interplay of synchronization and cortical input in models of brain networks

It is well known that synchronization patterns and coherence have a major role in the functioning of brain networks, both in pathological and in healthy states. In particular, in the perception of sound, one can observe an increase in coherence between the global dynamics in the network and the auditory input. In this perspective article, we show that synchronization scenarios are determined by a fine interplay between network topology, the location of the input, and frequencies of these cortical input signals. To this end, we analyze the influence of an external stimulation in a network of FitzHugh-Nagumo oscillators with empirically measured structural connectivity, and discuss different areas of cortical stimulation, including the auditory cortex.

==> SAW23_arxiv <==
\begin{thebibliography}{10}
\providecommand{\MR}{\relax\unskip\space MR }
\providecommand{\url}[1]{\normalfont{#1}}
\providecommand{\urlprefix}{Available at }

\bibitem{ABR04}
D. Abrams and S. Strogatz, \emph{Chimera states for coupled oscillators}, Phys. Rev. Lett. 93 (2004), p. 174102.

\bibitem{BAD13}
R. Bader, \emph{Nonlinearities and Synchronization in Musical Acoustics and Music Psychology}, Springer, Berlin, 2013.

\bibitem{BAD20}
R. Bader, \emph{Neural coincidence detection strategies during perception of multi-pitch musical tones}, arXiv:2001.06212v1  (2020).

\bibitem{BAS18}
D. Bassett, P. Zurn, and J. Gold, \emph{On the nature and use of models in network neuroscience}, Nat. Rev. Neurosci. 19 (2018), pp. 566--578.

\bibitem{BOC18}
S. Boccaletti, A. Pisarchik, C. del  Genio, and A. Amann, \emph{Synchronization: {F}rom Coupled Systems to Complex Networks}, Cambridge University Press, Cambridge, 2018.

\bibitem{BOH09}
J. Bohland, C. Allen, and P. Mitra, \emph{The brain atlas concordance problem: {Q}uantitative comparison of anatomical parcellations}, PLOS ONE 4 (2009), p. e7200.

\bibitem{CHE07a}
A. Chernihovskyi and K. Lehnertz, \emph{Measuring synchronization with nonlinear excitable media}, Int. J. Bifurc. Chaos 17 (2007), pp. 3425--3429.

\bibitem{CHE05e}
A. Chernihovskyi, F. Mormann, M. M{\"u}ller, C. Elger, G. Baier, and K. Lehnertz, \emph{{EEG} analysis with nonlinear excitable media}, J. Clin. Neurophysiol. 22 (2005), pp. 314--329.

\bibitem{CON23}
M. Contreras, E. Medeiros, A. Zakharova, P. H{\"o}vel, and I. Franovi{\'c}, \emph{Scale-free avalanches in arrays of {F}itz{H}ugh-{N}agumo oscillators}, Chaos 33 (2023), p. 093106.

\bibitem{EVA12}
A. Evans, A. Janke, D. Collins, and S. Baillet, \emph{Brain templates and atlases}, NeuroImg 62 (2012), pp. 911--922.

\bibitem{FIT61}
R. FitzHugh, \emph{Impulses and physiological states in theoretical models of nerve membrane}, Biophys. J. 1 (1961), pp. 445--466.

\bibitem{FRA18b}
I. Franovi{\'c} and V. Klinshov, \emph{Stimulus-evoked activity in clustered networks of stochastic rate-based neurons}, Eur. Phys. J. Spec. Top. 227 (2018), pp. 1063--1076.

\bibitem{GER20}
M. Gerster, R. Berner, J. Sawicki, A. Zakharova, A. Skoch, J. Hlinka, K. Lehnertz, and E. Sch{\"o}ll, \emph{{FitzHugh-Nagumo} oscillators on complex networks mimic epileptic-seizure-related synchronization phenomena}, Chaos 30 (2020), p. 123130.

\bibitem{HAR20a}
L. Hartmann and R. Bader, \emph{Neural synchronization of music large-scale form}, arXiv:2005.06938v1  (2020).

\bibitem{HOU20a}
Y. {Hou}, B. Song, Y. Hu, Y. Pan, and Y. Hu, \emph{The averaged inter-brain coherence between the audience and a violinist predicts the popularity of violin performance}, NeuroImage 211 (2020), p. 116655.

\bibitem{JOR94}
P. Joris, L. Carney, P. Smith, and T. Yin, \emph{Enhancement of {N}eural {S}ynchronization in the {A}nteroventral {C}ochlear {N}ucleus. {I}. {R}esponses to {T}ones at the {C}haracteristic {F}requency}, J. Neurophysiol. 71 (1994), p. 1022.

\bibitem{KIM18}
H. Kim, J. Moon, G. Mashour, and U. Lee, \emph{Mechanisms of hysteresis in human brain networks during transitions of consciousness and unconsciousness: theoretical principles and empirical evidence}, PLoS Comput. Biol. 14 (2018), p. e1006424.

\bibitem{KOE13}
S. Koelsch, M. Rohrmeier, R. Torrecuso, and S. Jentschke, \emph{Processing of hierarchical syntactic structure in music}, Proc. Natl. Acad. Sci. U.S.A. 110 (2013), p. 15443.

\bibitem{KUR02a}
Y. Kuramoto and D. Battogtokh, \emph{{Coexistence of Coherence and Incoherence in Nonlocally Coupled Phase Oscillators.}}, Nonlin. Phen. in Complex Sys. 5 (2002), pp. 380--385.

\bibitem{LAR15a}
E. Large, J. Herrera, and M. Velasco, \emph{Neural {N}etworks for {B}eat {P}erception in {M}usical {R}hythm}, Front. Neurosci. 9 (2015), p. 159.

\bibitem{MAS15a}
P. Massobrio, L. de  Arcangelis, V. Pasquale, H. Jensen, and D. Plenz, \emph{Criticality as a signature of healthy neural systems}, Front. Syst. Neurosci. 9 (2015), p.~22.

\bibitem{NAG62}
J. Nagumo, S. Arimoto, and S. Yoshizawa., \emph{An active pulse transmission line simulating nerve axon.}, Proc. IRE 50 (1962), pp. 2061--2070.

\bibitem{OME13}
I. Omelchenko, O. Omel'chenko, P. H{\"o}vel, and E. Sch{\"o}ll, \emph{When nonlocal coupling between oscillators becomes stronger: patched synchrony or multichimera states}, Phys. Rev. Lett. 110 (2013), p. 224101.

\bibitem{PET13}
S. Petkoski, D. Iatsenko, L. Basnarkov, and A. Stefanovska, \emph{Mean-field and mean-ensemble frequencies of a system of coupled oscillators}, Phys. Rev. E 87 (2013), p. 032908.

\bibitem{PET19}
S. Petkoski and V. Jirsa, \emph{Transmission time delays organize the brain network synchronization}, Phil. Trans. R. Soc. A 377 (2019), p. 20180132.

\bibitem{PIK01}
A. Pikovsky, M. Rosenblum, and J. Kurths, \emph{Synchronization: a universal concept in nonlinear sciences}, 1st ed., Cambridge University Press, Cambridge, 2001.

\bibitem{RIB10}
T.L. Ribeiro, M. Copelli, F. Caixeta, H. Belchior, D. Chialvo, M.A. Nicolelis, and S. Ribeiro, \emph{Spike avalanches exhibit universal dynamics across the sleep-wake cycle}, PloS One 5 (2010).

\bibitem{SAN15a}
P. Sanz-Leon, S. Knock, A. Spiegler, and V. Jirsa, \emph{Mathematical framework for large-scale brain network modeling in {T}he {V}irtual {B}rain}, Neuroimage 111 (2015), pp. 385--430.

\bibitem{SAW20}
J. Sawicki, \emph{Delay controlled partial synchronization in complex networks}, Springer Theses, Springer, Heidelberg, 2019.

\bibitem{SAW18a}
J. Sawicki, M. Abel, and E. Sch{\"o}ll, \emph{Synchronization of organ pipes}, Eur. Phys. J. B 91 (2018), p.~24.

\bibitem{SAW23a}
J. Sawicki, R. Berner, S. Loos, M. Anvari, R. Bader, W. Barfuss, N. Botta, N. Brede, I. Franovi{\'c}, D. Gauthier, S. Goldt, A. Hajizadeh, P. H{\"o}vel, O. Karin, P. Lorenz-Spreen, C. Miehl, J. M{\"o}lter, S. Olmi, E. Sch{\"o}ll, A. Seif, P. Tass, G. Volpe, S. Yanchuk, and J. Kurths, \emph{Perspectives on adaptive dynamical systems}, Chaos 33 (2023), p. 071501.

\bibitem{SAW22}
J. Sawicki, L. Hartmann, R. Bader, and E. Sch{\"o}ll, \emph{Modelling the perception of music in brain network dynamics}, Front. Netw. Physiol. 2 (2022), p. 910920.

\bibitem{SAW21a}
J. Sawicki and E. Sch{\"o}ll, \emph{Influence of sound on empirical brain networks}, Front. Appl. Math. Stat. 7 (2021), p. 662221.

\bibitem{SCA18}
S. Scarpetta, I. Apicella, L. Minati, and A. de  Candia, \emph{Hysteresis, neural avalanches, and critical behavior near a first-order transition of a spiking neural network}, Phys. Rev. E 97 (2018), p. 062305.

\bibitem{SCH18k}
A. Schneider, \emph{Pitch and Pitch Perception}, 1st ed., Springer Handbooks, Springer, Heidelberg, 2018.

\bibitem{SCH21}
E. Sch{\"o}ll, \emph{Partial synchronization patterns in brain networks}, Europhys. Lett. 136 (2021), p. 18001.

\bibitem{SHA20}
J. {Shainline}, \emph{Fluxonic processing of photonic synapse events}, IEEE J. Sel. Top. Quantum Electron. 26 (2020), p. 7700315.

\bibitem{SHI22}
J. Shi, K. Kirihara, M. Tada, M. Fujioka, K. Usui, D. Koshiyama, T. Araki, L. Chen, K. Kasai, and K. Aihara, \emph{Criticality in the healthy brain}, Front. Netw. Physiol. 1 (2022), p. 755685.

\bibitem{SIN18}
W. Singer, \emph{Neuronal oscillations: unavoidable and useful?}, Eur. J. Neurosci. 48 (2018), pp. 2389--2398.

\bibitem{SKO22}
A. Skoch, B. Rehak~Buckova, J. Mares, J. Tintera, P. Sanda, L. Jajcay, J. Horacek, F. Spaniel, and J. Hlinka, \emph{Human brain structural connectivity matrices-ready for modelling}, Scientific Data 9 (2022), p. 486.

\bibitem{STE10a}
A. Steyn-Ross and M. Steyn-Ross, \emph{Modeling phase transitions in the brain}, Vol. 509, Springer, Berlin, 2010.

\bibitem{TAS98}
P. Tass, M. Rosenblum, J. Weule, J. Kurths, A. Pikovsky, J. Volkmann, A. Schnitzler, and H. Freund, \emph{Detection of n:m phase locking from noisy data: Application to magnetoencephalography}, Phys. Rev. Lett. 81 (1998), p. 3291.

\bibitem{TZO02}
N. Tzourio-Mazoyer, B. Landeau, D. Papathanassiou, F. Crivello, O. Etard, N. Delcroix, B. Mazoyer, and M. Joliot, \emph{Automated anatomical labeling of activations in {SPM} using a macroscopic anatomical parcellation of the {MNI MRI} single-subject brain}, Neuroimage 15 (2002), pp. 273--289.

\bibitem{WIL19}
J. Wilting and V. Priesemann, \emph{25 years of criticality in neuroscience - established results, open controversies, novel concepts}, Curr. Opin. Neurobiol. 58 (2019), pp. 105--111.

\bibitem{ZAK20}
A. Zakharova, \emph{Chimera Patterns in Networks: Interplay between Dynamics, Structure, Noise, and Delay}, Understanding Complex Systems, Springer, Cham, 2020.

\end{thebibliography}

